Counterfactual Prediction Under Selective Confounding

This research addresses the challenge of conducting interpretable causal inference between a binary treatment and its resulting outcome when not all confounders are known. Confounders are factors that have an influence on both the treatment and the outcome. We relax the requirement of knowing all confounders under desired treatment, which we refer to as Selective Confounding, to enable causal inference in diverse real-world scenarios. Our proposed scheme is designed to work in situations where multiple decision-makers with different policies are involved and where there is a re-evaluation mechanism after the initial decision to ensure consistency. These assumptions are more practical to fulfill compared to the availability of all confounders under all treatments. To tackle the issue of Selective Confounding, we propose the use of dual-treatment samples. These samples allow us to employ two-step procedures, such as Regression Adjustment or Doubly-Robust, to learn counterfactual predictors. We provide both theoretical error bounds and empirical evidence of the effectiveness of our proposed scheme using synthetic and real-world child placement data. Furthermore, we introduce three evaluation methods specifically tailored to assess the performance in child placement scenarios. By emphasizing transparency and interpretability, our approach aims to provide decision-makers with a valuable tool. The source code repository of this work is located at https://github.com/sohaib730/CausalML.

==> Sections/Solution_Overview.tex <==
\section{Solution Overview}
\label{sec:overview}
\begin{comment}
Estimating an accurate risk score $\nu_{a_1}(x)$ under a desired treatment with $T=a_1$ is a crucial task in many applications, such as healthcare or child placement, where the goal is to predict the outcome of a particular treatment However, finding such an estimator from observational data is challenging. The problem here is the \textit{Selective Confounding} and missing ground truth labels, i.e. potential outcome $Y_{a_1}$, for samples that were assigned other treatments with $T \neq a_1$. 

Standard practice is to train the model over the samples where ground truth  label $Y_{a_1}$ is available [9,68]. The estimator is given as $\omega_{a_1}(x) = \mathbb{E}(Y_{a_1}|X)$ which is only identifiable as $ \mathbb{E}(Y|X, T=a_1)$ when either of the two conditions is valid: 1) All confounders are observed such that $Y_{a_1} \perp T | X$, or 2) in case of Randomized controlled trials when the probability of assignment to any treatment is equally likely resulting in $Y_{a_1} \perp T$. However, for the given problem setting none of the conditions is true. Thus, training over a subpopulation with available ground truth label $\tilde{\omega}_{a_1}(x) = \hat{\mathbb{E}}(Y|X, T=a_1)$ will not identify the accurate counterfactual quantity. Since it will underestimate the risk in cases where desired treatment has been historically assigned to lower-risk cases $E(Y|X, T=a_1) = E(Y_{a_1}|X, T=a_1) < E(Y_{a_1}|X)$ \cite{Coston_DR}.

Our solution to overcome confounding bias during training is to leverage dual-treatment samples. The exact definition of such samples is provided in Section \ref{sec:setup}. The intuition behind our solution is that if potential outcome $\hat{Y}_{a_1}$ is either known or estimated just for dual-treatment samples, the outcome estimator $\mu_{a_1}(x,z)$ is identifiable with no confounding bias as $\mathbb{E}(\hat{Y}_{a_1}|X,Z) = \mathbb{E}(\hat{Y}_{a_1}|X,Z,T=a_3)$. Similarly, conditional propensity score estimator $\pi_{a_3|\neq a_1}$  is identifiable without any bias over \textit{dual-treatmeent} subpopulation  by $\pi_{T=a_3|T \neq a_1}(X, Z)= P(T=a_3|X= x, Z=z,T \neq a_1)$ . These two nuisance estimators $\hat{\mu}_{a_1}(x,z),\hat{\pi}_{a_3|\neq a_1}(x,z)$ with no confounding bias can eventually be used to train target estimator $\hat{\nu}_{a_1}(x)$. The detailed algorithms are provided in Section \ref{sec:two-step method}.
\end{comment}
Our proposed solution aims to accurately estimate the risk score $\nu(x)$ for a desired treatment $a_1$ in the presence of selective confounding. Also, counterfactual learning is challenging due to missing ground truth labels, which is potential outcome $Y_{a_1}$, for samples with other treatments $T \neq a_1$.







 
 
\begin{comment}
It's possible depending how dual treatment samples have been defined. In child welfare application, dual treatment samples are those where children are reunited with their family within 30 days.  It can be argued that such short separation has no effect over the final outcome, meaning potential outcome are similar $Y_a = Y_{a'}$. However, it might not be possible to reduce the 30 days  there is trade off between number of dual treatment samples and difference between two potential outcomes.

For that purpose, it's important to see how dual treatment samples have been defined.
Since, it mainly depends on the application and definition of dual treatment samples. In child welfare application, dual treatment samples are those where children are reunited with their family within 30 days.  It can be argued that such short separation has no effect over the final outcome, meaning potential outcome are similar $Y_a = Y_{a'}$.

We propose a solution to learn both first stage estimators with no confounding loss. The idea is to use samples with dual treatment instead of proposed treatment to train the first stage estimators. It's ideal due to following reasons: 1 - No hidden confounders. 2 - Good distributional overlap with samples from other treatments because dual treatment samples usually lies at the boundary of decision policy. 3 - The potential outcome under dual treatment can be calibrated to represent proposed treatment.

 
\begin{align*}
    &\tau(X,Z) = E(Y_a'|X,Z)-E(Y_a|X,Z) & \text{(CATE)}\\
    &E_{X,Z}(\tau(X,Z)) = E(Y_{a'}) - E(Y_a) & \text{(ATE)}
\end{align*}
We can rewrite $\hat{\mu_a}(X,Z) = E(Y_a|X,Z)$ as $\hat{\mu_a}(X,Z) = E(Y_a' -\tau|X,Z)= E(Y|T=a',V,Z) + E(\tau)$. It enables us to train regressor function over dual treatment $T=a'$ and during prediction calibrate its outcome with ATE to estimate $\hat{\mu_a}(X,Z)$. 
\end{comment}







\begin{comment}
The procedure to imitate RCT and eventually estimation of ATE is presented in Algorithm 1. It first consider one sub-population representing DP lets say $dp_1$. Train one-class classifier to identify samples belongs to $T=a'$ or $T=1-a$. Now if samples in other sub-populations $dp_2,dp_3$ that received dual treatment $a'$ give very low probability for that one-class classifier? It means these units resemble to samples that have received treatment $T=a$ under $dp_1$ DP as shown in Figure 1b. Hence, for $dp_1$ we have identified dual treatment $T=a'$ samples calling them \textit{outliers} that covers same distribution as its samples that received $T=a$. We further find identical samples between samples with $T=a$ in $dp_1$ and outliers using k-nearest neighbors. Finally, we put both outliers samples and its corresponding samples with $T=a$ in $dp_1$ into global pool. From outliers we get factual outcome $Y_{a'}$ and $Y_a$ that received treatment $T=a$. The same procedure is repeated for all sub-poulations with different DPs, and the global pool will contain the samples that imitate RCT between treatment $a,a'$. Final, ATE between two treatments can be estimated empirically.

It can be argued that CATE might be more accurate choice of calibration instead of ATE. In case of, known confounding features, CATE can be estimated by training two regressors over both treatments i.e. $\tau(X,Z) = E(Y|T=a',V,Z)-E(Y|T=a,X,Z)$ The problem here is the confounded data under treatment $T=a$. Also, it leads to the same problem that we are trying to solve in a first place which is to avoid desired treatment samples.


\begin{algorithm}
\caption{Average Treatment Effect Estimation}
\label{alg:ATE}
\begin{algorithmic}
\For {each d $\in$ Decision Policies (DP)}
\State {Train estimator $P_d$ by regressing $\mathbb{I}(T=a',1-a) \sim X,Z|T=a',1-a$} 
\State Outliers = \{\}
\For {each $d' \in$ DP such that $d \neq d'$}
\For {each unit $(y,x,z|T=a')\ \in d'$}
\If{$P_d(T=a',1-a)|x,z) \approx 0$}
\State {Outliers = Outliers  $\cup\ (y,x,z,T=a')$}
\EndIf
\EndFor
\EndFor
\State {RCT = \{\}}
\For {each $(y,x,z,t) \in$ Outliers}
\State {Find k-Nearest Neighbor $N_k(x)$ in sub population with $DP=d,T=a$}
\State { $\hat{y_a} = \frac{1}{K}\sum_{i \in N_K(x)}y_{i}$ }
\State {RCT = RCT $\cup\ (\hat{y_a}, T=a)$}
\State {RCT = RCT $\cup\ (y,T=a')$}
\EndFor
\EndFor
\State { $\hat{E}(\tau(x,z)) = \frac{1}{n}\sum_{i \in {RCT,T_i=a'}}y_i - \frac{1}{n}\sum_{i \in {RCT,T_i=a}}y_i$}
\end{algorithmic}
\end{algorithm}
\end{comment}



